Joint Probability Trees

We introduce Joint Probability Trees (JPT), a novel approach that makes learning of and reasoning about joint probability distributions tractable for practical applications. JPTs support both symbolic and subsymbolic variables in a single hybrid model, and they do not rely on prior knowledge about variable dependencies or families of distributions. JPT representations build on tree structures that partition the problem space into relevant subregions that are elicited from the training data instead of postulating a rigid dependency model prior to learning. Learning and reasoning scale linearly in JPTs, and the tree structure allows white-box reasoning about any posterior probability $P(Q|E)$, such that interpretable explanations can be provided for any inference result. Our experiments showcase the practical applicability of JPTs in high-dimensional heterogeneous probability spaces with millions of training samples, making it a promising alternative to classic probabilistic graphical models.

==> makros.tex <==
\RequirePackage{xcolor}

%----------------------------------------------------------------------
% custom pseudocode commands
\RequirePackage{algpseudocode}

\algnewcommand\Input{\item[\textbf{Input:}]}
\algnewcommand\Static{\item[\textbf{Static:}]}
\algnewcommand\InputP{\item[\phantom{\textbf{Input:}}]}
\algnewcommand\Output{\item[\textbf{Output:}]}
\algnewcommand\OutputP{\item[\phantom{\textbf{Output:}}]}
\algnewcommand\In{\textbf{in}\xspace}
\algnewcommand\Not{\textbf{not}\xspace}
\algnewcommand\Null{\textsc{Null}\xspace}
\algnewcommand\And{\textbf{and}\xspace}
\algnewcommand\Or{\textbf{or}\xspace}
\algnewcommand\Yield{\textbf{yield}\xspace}
\algnewcommand\Each{\textbf{each}\xspace}

%----------------------------------------------------------------------

% *** bar charts in tables!  ***
\definecolor{myblue}{RGB}{87,118,169}

% \tablechartbar takes 1 argument (length in mm) and creates 
% a bar of length $length without label
\newcommand*{\tablechartbar}[1]{
  \begin{minipage}[c]{\linewidth}
    \begin{tikzpicture}
      \draw (0pt,0pt) (\linewidth,6mm);
      \draw[fill=chaptercolorlight] (0.0,0.1) rectangle ({#1*\linewidth},4mm);
    \end{tikzpicture}
  \end{minipage}
}

% \brokentablechartbar takes 1 argument (label) and creates 
% a 4 cm long bar with label on right, interrupted by two white lines
\newcommand*{\brokentablechartbar}[1]{
  \begin{minipage}[c]{4.5cm}
    \begin{tikzpicture}
      \draw (0cm,0cm) (4.5,0.5);
      \draw[fill=chaptercolorlight!100,draw=none] (0.2,0.152) rectangle ({0.2+4.0},0.438);
      \draw[draw=white,thick] (3.2,0.15) -- (3.3,0.45);
      \draw[draw=white,thick] (3.3,0.15) -- (3.4,0.45);
      \draw[very thin,draw=white] (4.2,.2) 
            node[text width=0pt,
                 text height=0pt,
                 font=\scriptsize,
                 text width=2cm,
                 align=right,
                 text=white,
                 anchor=east] {#1};
    \end{tikzpicture}
  \end{minipage}
}

% \tablechartscale takes 5 arguments and creates a 4cm long horizontal 
% axis with 5 ticks and labels
\newcommand*{\tablechartscale}[5]{
  \begin{minipage}[c]{\linewidth}
    \begin{tikzpicture}
    %{\linewidth}
      \draw (0cm,0cm) (\linewidth,5mm);
      %\tikzstyle{scalelabel}=[draw=none,text width=0pt,text height=0pt,text=black!50,font=\scriptsize]
      %\tikzset{scalelabel/.style={draw,label={[fill=yellow]0:#1}}}
      \draw[draw=black!50] (0.,0.2) -- ({\linewidth},0.2cm); % horizontal line
      \draw[draw=black!50] (0.,0.2) -- (0.,0.3); % tick
      \draw[draw=black!50] ({.25\linewidth},0.2) -- ({.25\linewidth},0.3); % tick
      \draw[draw=black!50] ({.5\linewidth},0.2) -- ({.5\linewidth},0.3); % tick
      \draw[draw=black!50] ({.75\linewidth},0.2) -- ({.75\linewidth},0.3); % tick
      \draw[draw=black!50] ({\linewidth},0.2) -- ({\linewidth},0.3); % tick
      \draw[draw=black!50] (0,0.3) node[anchor=south west] {\tiny#1};
      \draw[draw=black!50] ({.25\linewidth}, 0.3) node[anchor=south] {\tiny#2};
      \draw[draw=black!50] ({.5\linewidth}, 0.3) node[anchor=south] {\tiny#3};
      \draw[draw=black!50] ({.75\linewidth}, 0.3) node[anchor=south] {\tiny#4};
      \draw[draw=black!50] ({\linewidth}, 0.3) node[anchor=south east] {\tiny#5};
    \end{tikzpicture}
  \end{minipage}
}

%----------------------------------------------------------------------
% et al. 
%----------------------------------------------------------------------
\newcommand{\etal}{\textit{et~al.}}

%----------------------------------------------------------------------
% cf
%----------------------------------------------------------------------
\newcommand{\cf}[1]{(cf.\ \citeauthor{#1}, \citeyear{#1})}

%----------------------------------------------------------------------
% TODO boxes
%----------------------------------------------------------------------
\newcommand{\todo}[1]{\textit{\textbf{\textcolor{red}{TODO: #1}}}}

%----------------------------------------------------------------------
% convenient predicate declarations, e.g. \pred{\foo} enables \foo(x)
%----------------------------------------------------------------------
\newcommand{\pred}[1]{\expandafter\def\csname #1\endcsname{\textit{#1}}}
\newcommand{\newpred}[2]{\expandafter\def\csname #1\endcsname{#2}}

\newcommand{\mlnpred}[1]{\expandafter\def\csname #1\endcsname{\textbf{#1}}}

%----------------------------------------------------------------------
% fix the spacings above formulas
%----------------------------------------------------------------------

\AtBeginDocument{%
 \abovedisplayskip=0pt plus 5pt minus 9pt
 \abovedisplayshortskip=0pt plus 3pt
 \belowdisplayskip=12pt plus 3pt minus 9pt
 \belowdisplayshortskip=7pt plus 3pt minus 4pt
}

%----------------------------------------------------------------------
% new column type -- with precpecified width but horizontally centered
%----------------------------------------------------------------------
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }

%----------------------------------------------------------------------
% \nopar command to suppress spacing before the next paragraph
%----------------------------------------------------------------------
%\let\svpar\par
%\edef\svparskip{\the\parskip}
%\def\revertpar{\svpar\setlength\parskip{\svparskip}\let\par\svpar}
%\def\nopar{\leavevmode\setlength\parskip{\svparskip}%
%\def\par{\svpar\let\par\revertpar}%
%\vspace{-\baselineskip}}


%----------------------------------------------------------------------
% calligraphic X -- set of possible worlds
%----------------------------------------------------------------------
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}

%----------------------------------------------------------------------
% calligraphic I -- interpretation of a logical KB 
%----------------------------------------------------------------------
\newcommand{\Ical}{\ensuremath{\mathcal{I}}\xspace}

%----------------------------------------------------------------------
% calligraphic M -- models of a sentence 
%----------------------------------------------------------------------
\newcommand{\Mcal}{\ensuremath{\mathcal{M}}\xspace}

%----------------------------------------------------------------------
% calligraphic D -- training data set 
%----------------------------------------------------------------------
\newcommand{\Dcal}{\ensuremath{\mathcal{D}}\xspace}

%----------------------------------------------------------------------
% calligraphic L -- lieklihood function
%----------------------------------------------------------------------
\newcommand{\Lcal}{\ensuremath{\mathcal{L}}\xspace}

%----------------------------------------------------------------------
% calligraphic N -- normal distribution
%----------------------------------------------------------------------
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}\xspace}

%----------------------------------------------------------------------
% Boolean set 
%----------------------------------------------------------------------
\newcommand{\B}{\ensuremath{\mathds{B}}\xspace}

%----------------------------------------------------------------------
% implications 
%----------------------------------------------------------------------
\newcommand{\limpl}{\ensuremath{\rightarrow}}
\newcommand{\lbimpl}{\ensuremath{\leftrightarrow}}
\newcommand{\lentails}{\mathrel{|\!\!\!=}}

%----------------------------------------------------------------------
% real numbers
%----------------------------------------------------------------------
\newcommand{\R}{\ensuremath{\mathds{R}}}

%----------------------------------------------------------------------
% natural numbers
%----------------------------------------------------------------------
\newcommand{\N}{\ensuremath{\mathds{N}}}

%----------------------------------------------------------------------
% likelihood
%----------------------------------------------------------------------
\renewcommand{\l}{\ensuremath{\mathcal{L}}}

%----------------------------------------------------------------------
% log likelihood
%----------------------------------------------------------------------
\renewcommand{\ll}{\ensuremath{\mathcal{LL}}}

%----------------------------------------------------------------------
% pseudo likelihood
%----------------------------------------------------------------------
\newcommand{\pl}{\ensuremath{\mathcal{P\!L}}}

%----------------------------------------------------------------------
% pseudo log likelihood
%----------------------------------------------------------------------
\newcommand{\pll}{\ensuremath{\mathcal{P\!LL}}}

%----------------------------------------------------------------------
% markov blanket
%----------------------------------------------------------------------
\newcommand{\mb}{\textit{MB}}

%----------------------------------------------------------------------
% left and right angular brackets
%----------------------------------------------------------------------
\newcommand{\la}{\left<}
\newcommand{\ra}{\right>}

%----------------------------------------------------------------------
% left and right curly brackets
\newcommand{\lc}{\{}
\newcommand{\rc}{\}}

%----------------------------------------------------------------------
% brackets environment
%----------------------------------------------------------------------
\newcommand{\brackets}[1]{\left(#1\right)}

%----------------------------------------------------------------------
% (conditional) expectation
%----------------------------------------------------------------------
\newcommand{\E}[1]{\ensuremath{\mathds{E}\left(#1\right)}}
\newcommand{\Econd}[1]{\ensuremath{\mathds{E}\left(\begin{array}{c|c}#1\end{array}\right)}}

%----------------------------------------------------------------------
% functions
%----------------------------------------------------------------------
\newcommand{\F}[1]{\ensuremath{F\left(#1\right)}}
\newcommand{\f}[1]{\ensuremath{f\left(#1\right)}}
\newcommand{\Exp}[1]{\exp\left(#1\right)}
\newcommand{\Log}[1]{\log\left(#1\right)}
\newcommand{\fun}[2]{#1\left(#2\right)}

%----------------------------------------------------------------------
% (conditional) probability
%----------------------------------------------------------------------
\renewcommand{\P}[1]{\ensuremath{P\!\left(#1\right)}}
\newcommand{\Pcond}[2]{\ensuremath{\arraycolsep=1.ptP\!\left(\!\begin{array}{c|c}\begin{array}{c}#1\end{array} & \begin{array}{c}#2\end{array}\end{array}\!\right)}}

%----------------------------------------------------------------------
% without (set operator)
%----------------------------------------------------------------------
\newcommand{\wo}{\backslash}

%----------------------------------------------------------------------
% decorators
%----------------------------------------------------------------------
\newcommand{\xhat}{\ensuremath{\widehat{x}}}
\newcommand{\onebf}{\ensuremath{\mathbf{1}}}
\renewcommand{\models}{\vDash}

%----------------------------------------------------------------------
% \argmax and \argmin
%----------------------------------------------------------------------
\DeclareMathOperator*{\argmax}{\text{arg}\,\text{max}}
\DeclareMathOperator*{\argmin}{\text{arg}\,\text{min}}

%----------------------------------------------------------------------
% boldface and italic
%----------------------------------------------------------------------
\newcommand{\bfit}[1]{\textbf{\textit{#1}}}



